CHC-COMP 2023: Competition Report

CHC-COMP 2023 is the sixth edition of the Competition of Solvers for Constrained Horn Clauses. The competition was run in April 2023 and the results were presented at the 10th Workshop on Horn Clauses for Verification and Synthesis held in Paris, France, on April 23, 2023. This edition featured seven solvers (six competing and one hors concours) and six tracks, each of which dealing with a class of clauses. This report describes the organization of CHC-COMP 2023 and presents its results.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{Temur Kutsia, Daniel Ventura, David Monniaux \&\\
 Jos\'e F. Morales (Eds.): LSFA 2023 + HCVS 2023\\
EPTCS 402, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.402.10}{10.4204/EPTCS.402.10}}

